Effective Long-Context Scaling of Foundation Models

We present a series of long-context LLMs that support effective context windows of up to 32,768 tokens. Our model series are built through continual pretraining from Llama 2 with longer training sequences and on a dataset where long texts are upsampled. We perform extensive evaluation on language modeling, synthetic context probing tasks, and a wide range of research benchmarks. On research benchmarks, our models achieve consistent improvements on most regular tasks and significant improvements on long-context tasks over Llama 2. Notably, with a cost-effective instruction tuning procedure that does not require human-annotated long instruction data, the 70B variant can already surpass gpt-3.5-turbo-16k's overall performance on a suite of long-context tasks. Alongside these results, we provide an in-depth analysis on the individual components of our method. We delve into Llama's position encodings and discuss its limitation in modeling long dependencies. We also examine the impact of various design choices in the pretraining process, including the data mix and the training curriculum of sequence lengths -- our ablation experiments suggest that having abundant long texts in the pretrain dataset is not the key to achieving strong performance, and we empirically verify that long context continual pretraining is more efficient and similarly effective compared to pretraining from scratch with long sequences.

==> sections/pe_theory.tex <==
\subsection{PE Theory -- Igor}

\wh{@Igor, summarize the idea and remove the derivation to appendix?}

Basic idea: RoPE maps an embedding vector $x\in \mathbb R^d$ into a curve on a sphere in $\mathbb C^{d/2}$ parametrized by a real parameter $t\in \mathbb R$:

\begin{equation*}
f^{RoPE}(x, t)_j = \left(x_{2j} + i x_{2j+1}\right)e^{ib^{-\frac{2j}{d}}t}.    
\end{equation*}

The purpose of this mapping is to help the attention module to separate the vectors corresponding to two instances of the same token that are situated at different positions in the input sequence. 

Aiming at extending the sequence length from $N$ to $\hat N$ of a transformer pre-trained with a particular positional embedding $f,$ we would like to come up with a positional embedding $f$ that minimizes the distance between the new and the new images of the embedded vectors:
\[\max_{x\in \mathcal X}\min_{k\in \{0,..N\}~j\in \{0,..\hat N -1\}}\|f(x, k) - \hat f (x, j)\|,\]
where $\mathcal X \subset \mathbb R^d$ is the set of vectors that may need to be embedded.

With this in mind, we consider two different methods to extend the sequence length of a trained transformer: Position Interpolation (PI) parameterized with $\alpha$,  and Base Adjustment (BA) parameterized with $\beta.$ These two methods correspond to the following mappings:

\begin{align*} 
f^{RoPE+PI}(x,t)_j &= \left(x_{2j} +i x_{2j+1}\right)e^{i\alpha \cdot b^{-\frac{2j}{d}}t } \\
f^{RoPE+BA}(x,t)_j &= \left(x_{2j} + i x_{2j+1}\right)e^{i(\beta b)^{-\frac{2j}{d}}t}
\end{align*}

Comparing alternative positional embeddings $\hat f$ mapping $\mathbb R^d \times \mathbb N$ into $\mathbb C^{d/2},$ we should prefer the one with the maximal value of the distance betweeen the two closest images:
\[\min_{x\in \mathcal X; k\ne j \in \{0..\hat N-1\} }\|\hat f(x, k) - \hat f(x, j)\|.\]

% Since this metric is very difficult to compute in practice, we consider  $\min_{i\in \{0..N-1\}} \|f(x, i+1) - f(x, i)\|$ as the metric of interest, assuming that the curve in $\mathbb C^{d/2}$ does not have self-intersection within $t\in [0, N].$

While it is difficult to visualize a mapping $\mathbb R^d \times \mathbb N \to \mathbb C^{d/2},$ we can consider $x \in \mathbb R^d $ to be fixed and visualize the projection $\mathbb R \to \mathbb R^3.$ To get the intuition behind PI and BA, let us consider the helix that is formed by Re$\left[f^{RoPE}(x, t)_0\right]$, Im$\left[f^{RoPE}(x, t)_0\right]$ and Re$\left[f^{RoPE}(x, t)_j\right].$ The example on the Figure \ref{fig:RoPE} depicts a black helix line given with the system
\[x = \textrm{cos } t;
y = \textrm{sin } t;
z = \textrm{sin } at.\]
The red dots on the line correspond to $11$ integer values of $t.$ 

Figure \ref{fig:RoPE_PI} aims to illustrate the impact of Position Interpolation on the relative position of the mapped vectors. The distance between the consecutive points got reduced considerably compered to Figure \ref{fig:RoPE}. The impact of Base Adjustment is illustrated on Figure \ref{fig:RoPE_BA}. It could be seen that the distance between the consecutive points remained almost the same as on Figure \ref{fig:RoPE}, although the minimal distance between points got considerably reduced due to the increased frequency of the helix. The effect of increased frequency of the helix is reduced in the high dimension setting. The value of the coefficient $a$ for the helix depicted on Figure \ref{fig:RoPE} is two times larger than the value of the coefficient $a$ for the helix depicted on Figure \ref{fig:RoPE_BA}. If the dimension of the input of the attention mechanism is $d=128,$ then the difference between $\theta_1$ at $b=10,000$ and $\theta_1$ at $b=500,000$ is only $6\%.$

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1\linewidth]{sections/imgs/RoPE.pdf}
         \caption{RoPE}
         \label{fig:RoPE}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1\linewidth]{sections/imgs/RoPE+PI.pdf}
        \caption{RoPE+PI}
    \label{fig:RoPE_PI}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=1\linewidth]{sections/imgs/RoPE+BA.pdf}
        \caption{RoPE+BA}
    \label{fig:RoPE_BA}
     \end{subfigure}
\caption{Visualization}
\end{figure}
% https://colab.research.google.com/drive/1MXOPKAHkoXTKl8tRPhEXQ0Y9xWj0Ix4Z?usp=sharing

To make a formal comparison between Positional Interpolation and Base Adjustment, let us analytically compare the pairwise distances between the images given by $f^{RoPE+PI}$ and $f^{RoPE+BA}$ for consecutive integer values of $t$.

Under this assumption, we will measure the distance in terms of the cosine similarity metric:
\[\cos \angle (a, b) = \frac{Re \langle a, b\rangle}{\|a\|\|b\|}\]
$\langle f^{RoPE}(x, m), f^{RoPE}(x, n)\rangle = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)e^{ib^{-\frac{2j}{d}}(m-n)}$

$\langle f^{RoPE+PI}(x, m), f^{RoPE+PI}(x, n)\rangle = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)e^{ib^{-\frac{2j}{d}}\alpha(m-n)}$

$\langle f^{RoPE+BA}(x, m), f^{RoPE+BA}(x, n)\rangle = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)e^{ib^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}(m-n)}$






From this perspective, 

The number of values $\mathbb N$ that can fit onto a curve such that $\min > \varepsilon$ is finite since a sphere in $\mathbb C^{d/2}$ is a compact of a finite measure. 
Moreover, ... 
For example, if a model has been trained on 

Both PI (position interpolation) and BA (base augmentation) can be viewed as two alternative ways to increase the effective length of the available curve. One by re-parametrizing the curve itself (PI), the other by changing its geometry (BA).





$\langle f^{RoPE}(x, m), f^{RoPE}(x, n)\rangle = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)e^{ib^{-\frac{2j}{d}}(m-n)}$

$\langle f^{RoPE+PI}(x, m), f^{RoPE+PI}(x, n)\rangle = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)e^{ib^{-\frac{2j}{d}}\alpha(m-n)}$

$\langle f^{RoPE+BA}(x, m), f^{RoPE+BA}(x, n)\rangle = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)e^{ib^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}(m-n)}$





$\cos \angle (f^{RoPE}(x, m), f^{RoPE}(x, n)) = \frac{Re \langle f^{RoPE}(x, m), f^{RoPE}(x, n)\rangle}{\sum_{j=0}^{d-1} x_j^2} = \frac{\sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)\sin(b^{-\frac{2j}{d}}(m-n))}{\sum_{j=0}^{d-1} x_j^2} $

$\cos \angle (f^{RoPE+PI}(x, m), f^{RoPE+PI}(x, n)) = \frac{Re \langle f^{RoPE+PI}(x, m), f^{RoPE+PI}(x, n)\rangle}{\sum_{j=0}^{d-1} x_j^2} = \frac{\sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)\sin(b^{-\frac{2j}{d}}\alpha(m-n))}{\sum_{j=0}^{d-1} x_j^2} $

$\cos \angle (f^{RoPE+BA}(x, m), f^{RoPE+BA}(x, n)) = \frac{Re \langle f^{RoPE+BA}(x, m), f^{RoPE+BA}(x, n)\rangle}{\sum_{j=0}^{d-1} x_j^2} = \frac{\sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}(m-n))}{\sum_{j=0}^{d-1} x_j^2} $

Let's put $m=n+1$ to compare the distance between the two consecutive positional embedding of the same vector $x.$

$\|x\|^2 \cos \angle (f^{RoPE+PI}(x, n+1), f^{RoPE+PI}(x, n)) = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)\sin(b^{-\frac{2j}{d}}\alpha)$

$\|x\|^2 \cos \angle (f^{RoPE+BA}(x, n+1), f^{RoPE+BA}(x, n)) = \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}})$

$\sum_{j=0}^{\frac{d}{2}-1}\min_k x_k^2\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}) \le \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}) \le \sum_{j=0}^{\frac{d}{2}-1}\max_k x_k^2\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}})$

$\min_k x_k^2 \sum_{j=0}^{\frac{d}{2}-1}\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}) \le \sum_{j=0}^{\frac{d}{2}-1}\left(x_{2j}^2 + x_{2j+1}^2\right)\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}) \le \max_k x_k^2 \sum_{j=0}^{\frac{d}{2}-1}\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}})$
$\frac{\min_k x_k^2}{\|x\|^2} \sum_{j=0}^{\frac{d}{2}-1}\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}}) \le \cos \angle (f^{RoPE+BA}(x, n+1), f^{RoPE+BA}(x, n)) \le \frac{\max_k x_k^2}{\|x\|^2} \sum_{j=0}^{\frac{d}{2}-1}\sin(b^{-\frac{2j}{d}}\beta^{-\frac{2j}{d}})$



Exploiting the symmetry in attention mechanism, let us assume that the embedding vector $x$ contains components of an approximately similar value and $\|x\| \propto \frac{d}{2}.$ Using that $\sin \theta \le \theta$ for $\theta \le 1$ and that $\sin \theta \approx \theta$ for $\theta \to 0, $ we can approximate

$\cos \angle (f^{RoPE}(x, n+1), f^{RoPE}(x, n)) \stackrel{\propto}{\approx} \frac{2}{d}\sum_{j=0}^{\frac{d}{2}-1} b^{-\frac{2j}{d}}=\frac{2(b-1)b^{\frac{2}{d}-1}}{d\left( b^{\frac{2}{d}-1} \right)}$

Considering the limit at $d\to \infty:$

$\lim_{d\to \infty}\cos \angle (f^{RoPE}(x, n+1), f^{RoPE}(x, n)) \stackrel{\propto}{\approx} \frac{b-1}{b\log b}\approx (\log b)^{-1}$

For $RoPE+BA$ the calculations are exactly the same, except for the substitution $b\to \beta b,$ thus

$\lim_{d\to \infty}\cos \angle (f^{RoPE+BA}(x, n+1), f^{RoPE+BA}(x, n)) \stackrel{\propto}{\approx} (\log b + \log \beta)^{-1}$

For $RoPE+PI,$ the multiplier $\alpha$ can be extracted from the summation sign at the sine  approximation step:

$\cos \angle (f^{RoPE+PI}(x, n+1), f^{RoPE+PI}(x, n)) \stackrel{\propto}{\approx} \frac{2}{d}\sum_{j=0}^{\frac{d}{2}-1} \alpha b^{-\frac{2j}{d}}=\alpha\frac{2(b-1)b^{\frac{2}{d}-1}}{d\left( b^{\frac{2}{d}-1} \right)}$

And thus

$\lim_{d\to \infty}\cos \angle (f^{RoPE+PI}(x, n+1), f^{RoPE+PI}(x, n)) \stackrel{\propto}{\approx} \alpha (\log b)^{-1}$



\subsection{Computing the length of the curve}

Assuming we were able to fit $N$ points on the curve, after the positional interpolation we can fit $N/\alpha.$ How much can we fit using base adjustment? What should be the value of $\beta$ for the new length to be $N/\alpha$ (for the same value of $T$?)

For a complex-valued curve $r(t): \mathbb R \to \mathbb C^{d/2},$ its length function can be computed as $l(T) = \int_0^T \|\frac{\partial}{\partial t} r(t)\|dt.$ Let us compute the derivative:

$\frac{\partial}{\partial t}f^{RoPE}(x, t)_j = ib^{-\frac{2j}{d}}\left(x_{2j} + i x_{2j+1}\right)e^{ib^{-\frac{2j}{d}}t}$

$\frac{\partial}{\partial t}f^{RoPE+PI}(x,t)_j = ib^{-\frac{2j}{d}}\alpha\left(x_{2j} +i x_{2j+1}\right)e^{ib^{-\frac{2j}{d}}t\alpha}$

$\frac{\partial}{\partial t}f^{RoPE+BA}(x,t)_j = ib^{-\frac{2j}{d}}\beta^{-j}\left(x_{2j} + i x_{2j+1}\right)e^{ib^{-\frac{2j}{d}}t\beta^{-j}}$

The norms:

$\|\frac{\partial}{\partial t}f^{RoPE}(x, t)\| = |\langle \frac{\partial}{\partial t}f^{RoPE}(x, t), \frac{\partial}{\partial t}f^{RoPE}(x, t)\rangle| = \sum_{j=0}^{\frac{d}{2}-1} b^{-\frac{4j}{d}}\left(x_{2j}^2 + x_{2j+1}^2\right)$

$\|\frac{\partial}{\partial t}f^{RoPE+PI}(x, t)\| = \alpha^2\sum_{j=0}^{\frac{d}{2}-1} b^{-\frac{4j}{d}}\left(x_{2j}^2 + x_{2j+1}^2\right)$

$\|\frac{\partial}{\partial t}f^{RoPE+BA}(x, t)\| =  \sum_{j=0}^{\frac{d}{2}-1} \beta^{-2j} b^{-\frac{4j}{d}}\left(x_{2j}^2 + x_{2j+1}^2\right)$

Since the norms do not have any dependency on $t,$ the length functions are proportional to the value of the argument $T.$ Thus, we can compare the methods $RoPE+PI$ and $RoPE+BA$ by comparing the marginal length information contained in the norms. Using the assumption on the embedding vector $x,$ we can approximate the norms as

$\|\frac{\partial}{\partial t}f^{RoPE}(x, t)\| \approx \sum_{j=0}^{\frac{d}{2}-1} b^{-\frac{4j}{d}} = \frac{b^2 - 1}{b^2(1-b^{-4/d})}\approx \frac{1}{1-b^{-4/d}}$

$\|\frac{\partial}{\partial t}f^{RoPE+PI}(x, t)\| \approx \sum_{j=0}^{\frac{d}{2}-1} b^{-\frac{4j}{d}} = \frac{b^2 - 1}{b^2(1-b^{-4/d})}\approx \frac{\alpha^2}{1-b^{-4/d}}$

$\|\frac{\partial}{\partial t}f^{RoPE+BA}(x, t)\| \approx \sum_{j=0}^{\frac{d}{2}-1} b^{-\frac{4j}{d}} = \frac{b^2 - 1}{b^2(1-b^{-4/d})}\approx \frac{1}{1-(b\beta^{\frac{d}{2}})^{-4/d}} = \frac{1}{1-b^{-4/d}\beta^{-2}}$

The two methods (RoPE+PI and RoPE+BA) should be comparable if the values of the parameters $\alpha$ and $\beta$ satisfy the relationship $\|\frac{\partial}{\partial t}f^{RoPE+PI}(x, t)\| = \|\frac{\partial}{\partial t}f^{RoPE+BA}(x, t)\|:$

$\alpha = \sqrt{\frac{1-b^{-4/d}}{1-b^{-4/d}\beta^{-2}}}$ or $\beta = \sqrt{\frac{\alpha^2b^{-4/d}}{\alpha^2-1+b^{-4/d}}}$


Plugging this back into the expression for $\lim_{d\to \infty}\cos \angle (f^{RoPE+PI}(x, n+1), f^{RoPE+PI}(x, n)) $ we get an expression that can be compared to the expression for $\lim_{d\to \infty}\cos \angle (f^{RoPE+BA}(x, n+1), f^{RoPE+BA}(x, n)) :$

$\lim_{d\to \infty}\cos \angle (f^{RoPE+PI}(x, n+1), f^{RoPE+PI}(x, n)) \stackrel{\propto}{\approx} \sqrt{\frac{1-b^{-4/d}}{1-b^{-4/d}\beta^{-2}}} (\log b)^{-1}$




==> sections/related_works.tex <==

% \subsection{Language Models}
% Language models are probabilistic distributions over word tokens, which have been widely studied and regarded as an important sign of progress in artificial intelligence \cite{matthew}. An important line of earlier works focused on statistical methods such as n-grams \cite{n_gram} and Hidden Markov Models \cite{hmm}. With the advance of deep neural networks, a bunch of architectures and techniques start to emerge that result in huge improvement on language modeling, starting from feed forward models \cite{ffn}, recurrent neural networks \cite{rnn}, LSTMs \cite{lstm, lstm_1}, and transformers \cite{transformers, transformers_1, transformers_2}. Among these, transformer networks become the choice of many large language models that scale up to billions of parameters because the self-attention mechanisms allow the models to reason over longer ranges and can take advantage of the massive parallelism and acceleration from modern hardwares. 

% \subsection{Retrieval-based LLMs}
% Despite highly effective, most transformer-based LLMs are having difficulties processing more tokens. One primary reason is that the vanilla self-attention is quadratic in the sequence length, which makes it both computationally difficult and memory-expensive to train and infer with low-latency. With the increasing interest and need of processing longer context, many works propose to endow LLMs with a external memory and a retrieval system \cite{retrieval-lm-tutorial} that gathers related documents from the input sequence. TODO: list a bunch of examples. 

\subsection{Long-context LLMs}
An external memory could potentially help LLMs as a decoupled retrieval system, but these LLMs might still require more fundamental improvements on their capabilities of digesting more information. 

Long LLaMA \cite{long_llama}, XGen from Saleforce \footnote{\url{https://blog.salesforceairesearch.com/xgen}}, ChatGPT \footnote{\url{https://openai.com/blog/chatgpt}} and GPT-4 \cite{gpt-4} from OpenAI, Claude family \footnote{\url{https://www.anthropic.com/index/introducing-claude}} from Anthropic and MPT-30B from Mosaic ML \footnote{\url{https://www.mosaicml.com/blog/mpt-30b}}. Lost in the middle \cite{lost_in_the_middle}, LongNet \cite{long_net}.

\subsection{Scaling and efficiency}



==> sections/short_task_improvements.tex <==
\subsection{How does Continual Pretraining with Longer Context Help with Short Tasks?}
\label{seqlen_analysis}

\wh{needs to improve this section or move to appendix}
In our experiments, a surprising observation is that continual pretraining with longer sequence length (i.e., from 4k to 16k/32k) can often improve the performance of many short tasks with minimal compute budget compared to the pretrain stage (\jy{add percentage}). To investigate the source of the improvements, we perform additional ablation by running continual pretraining without increasing the sequence length. 

% We study this potential benefits of long sequence continual pretraining rigorously in this section. We first continually pretrain \llamavtwo 7B from 4k to 32k context window with 8B tokens where we reinitialize the optimizer states. The reason to do so is that most \llama finetuning will follow this paradigm as the optimizer states are not publicly available. To figure out the potential influence of the optimizer rescheduling, we also launched another run where we fixed the context window to 4k (by adjusting the batch size accordingly to maintain the same training tokens) and keep everything else the same. Finally, we evaluate the performance of these two continual pretrain runs and compare them also with \llamavtwo. 

In Table \ref{table:seq_len_short_tasks}, we can see that 1) for most tasks, we get consistent improvements from relatively a few steps (5k) of continual pretraining and 2) the continual pretraining sequence length has little influence on most tasks. The starting learning rate of continual pretrain is $2e^{-5}$, which is a lot smaller than the ending learning rate $3e^{-5}$ of the pretrain stage. Therefore, we hypothesize that it is the smaller learning rate used in the continual pretraining that leads to the increasing performance of some short tasks, which also explains \jy{refer to the 70B results against LLama v2}. 

\begin{table}
  \small
  \centering
  \begin{adjustbox}{max width=1.2\linewidth, center}
  \begin{tabular}{lccccccc}
    \toprule
    % % all results 
    % Seq Len & Config & HumanEval & Math & GSM8K & MMLU & HellaSwag & TQA & SIQA & MBPP \\
    % \midrule
    % % 4k & \ding{55} & 12.804 & 3.288 & 13.950 & 45.292 & 75.931 & 64.752 & 48.414 \\
    % % 4k & \ding{51} & 15.854 & 2.967 & 16.755 & 46.603 & 76.887 & 65.989 & 48.618 \\
    % % 32k & \ding{51} & 15.244 & 3.609 & 16.224 & 46.304 & 76.628 & 66.715 & 49.181 \\
    % 4k & Llama 2 420k step & 14.02 & 3.14 & 13.27 & 44.18 & 75.81 & 63.32 & 48.87 & 20.2 \\
    % 4k & Llama 2 440k step & 15.85 & 2.72 & 14.17 & 44.76 & 76.27 & 64.72 & 48.20 & 22.2 \\
    % 4k & Llama 2 460k step & 17.07 & 3.42 & 14.56 & 46.62 & 76.07 & 64.70 & 48.46 & 22.8 \\
    % 4k & Llama 2 480k step & 12.80 & 3.29 & 13.95 & 45.29 & 75.93 & 64.75 & 48.41 & 22.2 \\
    % \midrule
    % 4k & + 20k step 3e-5->1e-5 & 16.46 & 3.11 & 14.18 & 46.24 & 76.63 & 65.80 & 48.87 & 23.4 \\
    % 4k & + 20k step 3e-5->3e-8 & 16.46 & 3.48 & 15.84 & 46.82 & 76.82 & 66.08 & 48.67 & 21.0\\
    % 4k & + 20k step 2e-5->2e-6 & 15.85 & 2.97 & 16.76 & 46.60 & 76.89 & 65.99 & 48.62 \\
    % 32k & + 20k step 2e-5->2e-6 & 15.24 & 3.61 & 16.22 & 46.30 & 76.63 & 66.72 & 49.18 \\


    Seq Len & Config & HumanEval & GSM8K & MMLU & TQA \\
    \midrule
    % 4k & \ding{55} & 12.804 & 3.288 & 13.950 & 45.292 & 75.931 & 64.752 & 48.414 \\
    % 4k & \ding{51} & 15.854 & 2.967 & 16.755 & 46.603 & 76.887 & 65.989 & 48.618 \\
    % 32k & \ding{51} & 15.244 & 3.609 & 16.224 & 46.304 & 76.628 & 66.715 & 49.181 \\
    4k & Llama 2 420k step & 14.02  & 13.27 & 44.18 & 63.32 \\
    4k & Llama 2 440k step & 15.85  & 14.17 & 44.76  & 64.72  \\
    4k & Llama 2 460k step & 17.07  & 14.56 & 46.62  & 64.70  \\
    4k & Llama 2 480k step & 12.80  & 13.95 & 45.29  & 64.75 \\
    \midrule
    4k & + 20k step 3e-5->1e-5 & 16.46 &  14.18 & 46.24 &  65.80  \\
    4k & + 20k step 3e-5->3e-8 & 16.46 &  15.84 & 46.82  & 66.08\\
    4k & + 20k step 2e-5->2e-6 & 15.85 &  16.76 & 46.60  & 65.99  \\
    32k & + 20k step 2e-5->2e-6 & 15.24 &  16.22 & 46.30 & 66.72 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \vspace{5pt}
  \caption{\textbf{Continual Pretrain Sequence Length on Short Tasks}: \jy{Maybe we can remove some tasks that do not differ too much in our main 70B results?}}
  \label{table:seq_len_short_tasks}
\end{table}


==> tables/pretrain_scrolls_evo.tex <==
\begin{table}
  \centering
  \begin{adjustbox}{max width=1.2\linewidth, center}
      \begin{tabular}{lrcccc}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Task Length} & NarrativeQA & Qasper & QuALITY & QMSum \\
        & & F1 & F1 & Acc & ROUGE-geo \\
        \midrule
        \multirow{4}{*}{\model 70B} & 4,096 & 27.5 & 28.9 & 46.0 & 10.9 \\
                                    & 8,192 & 28.7 & 32.7 & 50.4 & 11.9 \\
                                    & 12,288 & 30.2 & 35.1 & 53.7 & 14.4\\
                                    & 16,384 & 30.9 & 35.7 & 54.7 & 16.5 \\
        \bottomrule
      \end{tabular}
  \end{adjustbox}
  \vspace{5pt}
  \caption{\model's performance with different task lengths on the validation sets of SCROLLS. Our model can effectively leverage more context up to its training sequence length for all tasks. }
  \label{table:scrolls_context_length}
\end{table}

